Game-Theoretic Model of Incentivizing Privacy-Aware Users to Consent to Location Tracking

Nowadays, mobile users have a vast number of applications and services at their disposal. Each of these might impose some privacy threats on users' "Personally Identifiable Information" (PII). Location privacy is a crucial part of PII, and as such, privacy-aware users wish to maximize it. This privacy can be, for instance, threatened by a company, which collects users' traces and shares them with third parties. To maximize their location privacy, users can decide to get offline so that the company cannot localize their devices. The longer a user stays connected to a network, the more services he might receive, but his location privacy decreases. In this paper, we analyze the trade-off between location privacy, the level of services that a user experiences, and the profit of the company. To this end, we formulate a Stackelberg Bayesian game between the User (follower) and the Company (leader). We present theoretical results characterizing the equilibria of the game. To the best of our knowledge, our work is the first to model the economically rational decision-making of the service provider (i.e., the Company) in conjunction with the rational decision-making of users who wish to protect their location privacy. To evaluate the performance of our approach, we have used real-data from a testbed, and we have also shown that the game-theoretic strategy of the Company outperforms non-strategic methods. Finally, we have considered different User privacy types, and have determined the service level that incentivizes the User to stay connected as long as possible.

==> acks.tex <==
%\section{Acknowledgements}
%We would like to thank Tansu Alpcan for discussions we had on an earlier version of this paper.

==> authors.tex <==
\author{

\IEEEauthorblockN{
Emmanouil Panaousis\IEEEauthorrefmark{1},
Aron Laszka\IEEEauthorrefmark{2},
Johannes Pohl\IEEEauthorrefmark{3},\\
Andreas Noack\IEEEauthorrefmark{3}, 
and Tansu Alpcan\IEEEauthorrefmark{4}
}

\IEEEauthorblockA{
\IEEEauthorrefmark{1}
University of Brighton, UK}

\IEEEauthorblockA{
\IEEEauthorrefmark{2}
Institute for Software Integrated Systems, Vanderbilt University, Nashville, USA}

\IEEEauthorblockA{
\IEEEauthorrefmark{3}
University of Applied Sciences Stralsund, Germany}

\IEEEauthorblockA{
\IEEEauthorrefmark{4}
The University of Melbourne, Australia}
}
